Matching the Blanks: Distributional Similarity for Relation Learning

General purpose relation extractors, which can model arbitrary relations, are a core aspiration in information extraction. Efforts have been made to build general purpose extractors that represent relations with their surface forms, or which jointly embed surface forms with relations from an existing knowledge graph. However, both of these approaches are limited in their ability to generalize. In this paper, we build on extensions of Harris' distributional hypothesis to relations, as well as recent advances in learning text representations (specifically, BERT), to build task agnostic relation representations solely from entity-linked text. We show that these representations significantly outperform previous work on exemplar based relation extraction (FewRel) even without using any of that task's training data. We also show that models initialized with our task agnostic representations, and then tuned on supervised relation extraction datasets, significantly outperform the previous methods on SemEval 2010 Task 8, KBP37, and TACRED.

==> discussion.tex <==
\section{Discussion}
\label{sec:discussion}

Potential points of discussion:

\begin{itemize}
    \item Figure~\ref{fig:fewrel-limit-examples} shows that, given a limited budget
    of annotations, it is better to have a diverse set of relation types than large numbers
    of relations per type.
    
    \item Gap between the few-shot relation matching and the relation extraction tasks.
    Looking at the confusion matrix, it seems that the the most common error is flipping
    between "no relation" and the correct relation (or vice-versa). Modeling the
    \textsc{NIL} properly is likely to yield gains.
    
    \item We have not tried to increase, beyond two, the number of co-occuring entities to
    define statement equivalence.
    \item This work requires a entity linking annotations. It would be interesting to relax
    this requirement so that NER + heuristics based linking may be sufficient even if the result
    is noisy,  \textit{particularly if we require two entity mentions to co-occur within a 
    window of text}. (i.e., is mention ambiguity still a problem when considering "2-gram"
    entities?).
    \item 
\end{itemize}
